Bayesian Learning of Optimal Policies in Markov Decision Processes with Countably Infinite State-Space

Models of many real-life applications, such as queuing models of communication networks or computing systems, have a countably infinite state-space. Algorithmic and learning procedures that have been developed to produce optimal policies mainly focus on finite state settings, and do not directly apply to these models. To overcome this lacuna, in this work we study the problem of optimal control of a family of discrete-time countable state-space Markov Decision Processes (MDPs) governed by an unknown parameter $\theta\in\Theta$, and defined on a countably-infinite state space $\mathcal X=\mathbb{Z}_+^d$, with finite action space $\mathcal A$, and an unbounded cost function. We take a Bayesian perspective with the random unknown parameter $\boldsymbol{\theta}^*$ generated via a given fixed prior distribution on $\Theta$. To optimally control the unknown MDP, we propose an algorithm based on Thompson sampling with dynamically-sized episodes: at the beginning of each episode, the posterior distribution formed via Bayes' rule is used to produce a parameter estimate, which then decides the policy applied during the episode. To ensure the stability of the Markov chain obtained by following the policy chosen for each parameter, we impose ergodicity assumptions. From this condition and using the solution of the average cost Bellman equation, we establish an $\tilde O(dh^d\sqrt{|\mathcal A|T})$ upper bound on the Bayesian regret of our algorithm, where $T$ is the time-horizon. Finally, to elucidate the applicability of our algorithm, we consider two different queuing models with unknown dynamics, and show that our algorithm can be applied to develop approximately optimal control algorithms.

==> Regret.tex <==



 % \section{Regret analysis of \texorpdfstring{\Cref{alg:TSDE}}{Algorithm 1}} \label{sec:main_results}

\section{Regret analysis of \Cref{alg:TSDE}}\label{sec:main_results}

The performance of any learning policy $\pi_L$ is evaluated using the metric of expected regret compared to the optimal expected average cost of true parameter  $\boldsymbol{\theta}^*$, namely, $ J(\boldsymbol{\theta}^*)$.
In this section, we evaluate the performance of \Cref{alg:TSDE} and derive an upper bound for $R(T,\pi_{TSDE})$, its expected regret up to time $T$.
In \Cref{subsec:Preliminaries}, we argued that at time $t$ in  episode $k$ ($t_k \leq t < t_{k+1}$), there exist a constant $J(\theta_k)$ and a unique function $v(\cdot;\theta_k): \mathcal{X} \rightarrow\mathbb{R}$ such that $v\left(0^d;\theta_k\right)=0$ and
     \begin{equation} \label{eq:ACOE}
			J(\theta_k)+v(\boldsymbol X(t);\theta_k)= c(\boldsymbol X(t),\pi^*_{\theta_k}( \boldsymbol X(t)))+  \sum_{\boldsymbol y \in \mathcal{X}} P_{\theta_k}(\boldsymbol y | \boldsymbol X(t),\pi^*_{\theta_k}( \boldsymbol X(t))) 	v(\boldsymbol y;\theta_k),
		\end{equation}
	in which $\pi^*_{\theta_k}$ is the optimal or  best-in-class policy (depending on the context) according to parameter $\theta_k$ and $J(\theta_k)$ is the average cost for the Markov process obtained from MDP $\left(\mathcal{X},\mathcal{A},c,P_{\theta_k}\right)$ by following $\pi^*_{\theta_k}$. 
We derive a bound for the expected regret $R(T,\pi_{TSDE})$ following the proof steps of \cite{ouyang2017learning} while extending it to the countable state space setting of our problem.
Using  \eqref{eq:ACOE},  
the regret is decomposed into three terms and each term is bounded separately:
\begin{align}
 \label{eq:regret_decomposition}
		 R(T,\pi_{TSDE})&= \E \Big[\sum_{k=1}^{K_T} \sum_{t=t_k}^{t_{k+1}-1} c(\boldsymbol X(t),\pi^*_{\theta_k}( \boldsymbol X(t)))\Big]- T\E \left[J\left(\boldsymbol \theta^*\right)\right]=R_0+R_1+R_2,\\
		\text{with } R_0  = & \E\Big[ \sum_{k=1}^{K_T}T_k J(\theta_k) \Big]- T \E\Big[J(\boldsymbol\theta^*) \Big],\label{eq:R_0}
		\\
		R_1  = &\E\Big[\sum_{k=1}^{K_T}\sum_{t=t_k}^{t_{k+1}-1}  \Big[v(\boldsymbol X(t);\theta_k) -v(\boldsymbol X(t+1);\theta_k)\Big]\Big],\label{eq:R_1}\\
		R_2  = & \E\Big[\sum_{k=1}^{K_T}\sum_{t=t_k}^{t_{k+1}-1}  \Big[ 
v(\boldsymbol X(t+1);\theta_k)- \sum_{\boldsymbol y \in \mathcal{X}} P_{\theta_k}(\boldsymbol y | \boldsymbol X(t),\pi^*_{\theta_k}( \boldsymbol X(t))) 	v(\boldsymbol y;\theta_k)\Big] \Big].\label{eq:R_2}
	\end{align}
Before bounding the above regret terms, we address the complexities arising from the countable state space setting. 
Firstly, we need to study the maximum state (with respect to the $\ell_{\infty}$-norm) visited up to time $T$ in the MDP $\left(\mathcal{X},\mathcal{A},c,P_{\boldsymbol\theta^*}\right)$ following \Cref{alg:TSDE}; we denote this maximum state by $M^T_{\boldsymbol\theta^*}$. In \Cref{sec:max_hit_numbe_eps}, we derive upper bounds on the moments of hitting times of state $0^d$ and utilize this to bound the moments of random variable $M^T_{\boldsymbol\theta^*}$, which then lets us study the number of episodes $K_T$ by time $T$. 
Another challenge in analyzing the regret is that the relative value function $v(\boldsymbol x;\theta)$ is unlikely to be bounded in the countable state space setting. Hence, in \eqref{eq:bound_rel_val} and \eqref{eq:bound_rel_val_low}, we find bounds for the relative value function in terms of hitting time $\tau_{0^d}$ from any initial state $\boldsymbol x$. Based on these results, we provide an upper bound for the regret of \Cref{alg:TSDE} in \Cref{thm:main}.

\begin{Remark}
The skip-free to the right property in \Cref{assump:skipfrt} yields a polynomially-sized subset of the underlying state space that can be explored as a function of $T$. This polynomially-sized subset can be viewed as the effective finite-size of the system in the worst-case, and then, directly applying finite-state problem bounds \cite{ouyang2017learning} would result in a regret of order $\tilde O(T^{d+0.5})$; since $d\geq 1$, such a coarse bound is not helpful even for asserting asymptotic optimality. However, to achieve a regret of $\tilde O(\sqrt{T})$, it is essential to carefully understand and characterize the distribution of $M^T_{\boldsymbol \theta^*}$ and then its moments, as demonstrated in \Cref{lem:max_geom_rv}.
\end{Remark}
 

\textit{\bfseries Maximum state norm under polynomial and geometric ergodicity.} Here we state the results that characterize the maximum $l_\infty$-norm of the state vector achieved up until and including time $T$, and the resulting bounds on the number of episodes executed until time $T$. Owing to space constraints the details (including formal statements) are presented in \Cref{sec:proof_regret_analysis}. The results are listed as below: 
\begin{enumerate}[leftmargin=*]
    \item  In \Cref{lem:max_geom_rv}, we bound the moments of the maximum length of recurrence times of state $0^d$, denoted by $ \max_{1\leq i \leq T}  \tau_{0^d}^{(i)}$, using the ergodicity assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg}. This, along with the skip-free property, allows us to 
prove that the $p$-th moment of $ \max_{1\leq i \leq T}  \tau_{0^d}^{(i)}$ and $M^T_{\boldsymbol\theta^*}$ are both of order $O(\log^p T)$.
\item In \Cref{lem:number_macro_episodes}, we find an upper bound for the number of episodes in which the second stopping criterion is met or there exists a state-action pair for which $N_t(\boldsymbol x,a)$ has increased more than twice.
\item In \Cref{lem:number_episodes}, we  bound  the total number of episodes $K_T$ by time $T$ by bounding the number of episodes triggered by the first stopping criterion, using the fact that in such episodes, $\tilde{T}_k = \tilde{T}_{k-1}+1$. Moreover, to account for the settling time of each episode, we use geometric ergodicity and \Cref{lem:max_geom_rv}. It then follows that the expected value of the number of episodes $K_T$ is of the order $\tilde O(\sqrt{|\mathcal A|T})$.
\end{enumerate}



\textit{\bfseries Regret analysis.} Next, we bound regret terms $R_0$, $R_1$ and $R_2$ using the approach of \cite{ouyang2017learning} along with additional arguments to extend their result to a countably infinite state space. We consider the relative value function $v(\boldsymbol x;\theta)$ of policy  $\pi^*_{\theta}$ introduced for the optimal policy in ACOE or for the best in-class policy in the Poisson equation. In either of these cases, policy  $\pi^*_{\theta}$ satisfies  \eqref{eq:ACOE_case2}, which  is the corresponding Poisson equation with forcing function ${c}(\boldsymbol x,\pi^*_{\theta}(\boldsymbol x))$ in a Markov chain with transition matrix $P_{\theta}^{\pi^*_{\theta}}$. 
In \eqref{eq:PoissonEq}, we presented the solution $(J,v)$ to the Poisson equation, which yields the following upper bound for the relative value function, as argued in \Cref{subsec:exist_pois_eqn}:
\begin{equation} \label{eq:bound_rel_val}
     v(\boldsymbol x;\theta)\leq \bar{C}^{\pi^*_{\theta}}(\boldsymbol x) \leq  \mathbb{E}^{\pi^*_{\theta}}_{\boldsymbol x}\left[  Kd  \left(\norm{\boldsymbol x}_{\infty}+h\tau_{0^d}\right)^r \tau_{0^d}\right].
\end{equation}
We can similarly lower bound the relative value function using \Cref{assump:sup_J_V} as
\begin{align} \label{eq:bound_rel_val_low}
     v(\boldsymbol x;\theta)\geq - J(\theta) \mathbb{E}^{\pi^*_{\theta}}_{\boldsymbol x}[\tau_{0^d}]\geq - J^* \mathbb{E}^{\pi^*_{\theta}}_{\boldsymbol x}[\tau_{0^d}].
\end{align}
From \Cref{assump:geom_erg}, all moments of $\tau_{0^d}$ and thus, the derived bounds are finite. Also, in \Cref{lem:hitting_time} we bound the moments of  $\tau_{0^d}$ of order $i=1,\ldots,r+1$ using the polynomial Lyapunov function $V^p_{\theta_1,\theta_2}$, which is then used to bound the expected regret.  We next bound the first regret term $R_0$ from the first stopping criterion in terms of the number of episodes $K_T$ and the settling time of each episode $k$. 


\begin{Lemma}\label{lem:R_0_bound}
	The first regret term $R_0$ satisfies 
 $R_0 \leq   J^*  \E[K_T(\max_{1\leq i  \leq T} \tau_{0^d}^{(i)}+1)].$
\end{Lemma}
Proof of \Cref{lem:R_0_bound} is given in \Cref{subsec:R_0_bound}.  From \Cref{lem:max_geom_rv}, moments of $\max_{1\leq i  \leq T} \tau_{0^d}^{(i)}$ are bounded by polylogarithmic functions. Futhermore, as a result of \Cref{lem:number_episodes}, expected value of the number of episodes $K_T$ is of the order $\tilde O (\sqrt{|\mathcal A|T})$, which leads to a $\tilde O (J^*\sqrt{|\mathcal A|T})$ regret term $R_0$. Next, an upper bound on $R_1$ defined in \eqref{eq:R_1} is derived.
In the proof of \Cref{lem:R_1_bound} we argue that as the relative value function is equal to $0$ at all time instances $t_k$ for $k \leq K_T$, the only term that contributes to the regret is the value function at the end of time horizon $T$. We use the lower bound derived in \eqref{eq:bound_rel_val_low} to show that  the second regret term $R_1$ is $\tilde O (1)$; the proof is given in \Cref{subsec:R_1_bound}. 
\begin{Lemma}\label{lem:R_1_bound}
The second regret term $R_1$ satisfies 
 $ R_1 \leq c_2 \E [( M^T_{\boldsymbol\theta^*})^{r_*^p}]+c_3$, where $c_2={J^*2^{r_*^p} s_*^p}(\beta^p_*)^{-1} $ and $c_3={J^*}(\beta^p_*)^{-1}\Big( s_*^p \left(2h\right)^{r_*^p} + {b^p_{*}}(K_*)^{-1}\Big)$. 
\end{Lemma}
From \Cref{lem:max_geom_rv}, $\E[( M^T_{\boldsymbol\theta^*})^{r_*^p}]$ is $O(\log^{r_*^p} T)$; hence, $R_1$ is upper bounded by a polylogarithmic function of the order $r_*^p$. Finally, in \Cref{lem:R_2_bound}, we derive an upper bound for the third regret term $R_2$ defined in \eqref{eq:R_2}
 using the bound derived for the relative value function in \eqref{eq:bound_rel_val}. To bound $R_2$, we characterize it in terms of the difference between the empirical and true unknown transition kernel and following the concentration method used in \cite{weissman2003inequalities,auer2008near,ouyang2017learning,akbarzadeh2022learning}, we argue that with high probability the total variation distance between the two distributions is small; for
proof, see \Cref{subsec:R_2_bound}.

\begin{Lemma}\label{lem:R_2_bound}
	For a problem-dependent constant $c_{p_3}$ and polynomial $Q(T)= c_{p_3} (Th)^{r+r_*^p}/48$, the second regret term $R_2$ satisfies  
\begin{align*}
    R_2 
    &\leq    (\log (hT+h)+1)^d + c_{p_3}\sqrt{|\mathcal A| T }\log_2 \left({ 2|\mathcal A|T^2Q(T) }\right)\E\Big[   {(M^T_{\boldsymbol\theta^*}+h)^{d+r+r_*^p}}\Big(\max_{1\leq i  \leq T} \tau_{0^d}^{(i)} \Big)\Big].
\end{align*}
\end{Lemma}
\begin{Remark}
 By problem-dependent parameters, we refer to the parameters that characterize the complexity or size of the model class $\Theta$. These parameters are not just a function of the size of the state space and diameter of the MDP (as mentioned in the literature on finite-size problems\cite{agrawal2017optimistic,gopalan2015thompson,ouyang2017learning}), as stability needs to be accounted for in the countable state space setting. The dependence is, thus, more complex and requires the inclusion of stability parameters, such as Lyapunov functions, petite sets, and ergodicity coefficients that are discussed in Assumptions \ref{assump:costfn}-\ref{assump:sup_J_V}.
\end{Remark}

\SAcomment{The above Lemma results in a $\tilde O(Kr d J^* h^{d+2r+r_*^p}\sqrt{|\mathcal A| T })$ regret term as a result of  \Cref{lem:max_geom_rv}, where  $h$ is the skip-free parameter defined in \Cref{assump:skipfrt}, $d$ is the dimension of the state space,  $K$ and $r$ are the cost function parameters defined in \Cref{assump:costfn},  $J^*$ is the supremum on the optimal cost,  $r_*^p$ is defined in \Cref{assump:poly_erg}, and where $\tilde O$ hides logarithmic factors in problem parameters one of which is $\log^{d+r+r_*^p+2}(T)$. For simplicity, we have not included the Lyapunov functions related parameters in the regret. Finally, from Lemmas \ref{lem:R_0_bound}, \ref{lem:R_1_bound}, \ref{lem:R_2_bound}, along with the Cauchy-Schwarz inequality, we conclude that the regret of \Cref{alg:TSDE} $R(T,\pi_{TSDE})(=R_0+R_1+R_2)$ is $\tilde O(Kr d J^* h^{d+2r+r_*^p}\sqrt{|\mathcal A| T })$; for brevity, we will state that regret is of the order $\tilde O(dh^d\sqrt{|\mathcal A|T})$.}
\begin{Theorem} \label{thm:main}
Under Assumptions \ref{assump:costfn} through \ref{assump:sup_J_V},	the regret of \Cref{alg:TSDE}, $R(T,\pi_{TSDE})$ is $\tilde O(d\sqrt{|\mathcal A|T})$.
\end{Theorem}
\Cref{thm:main} can be extended to the problem of finding the best policy within a sub-class of policies in set $\Pi$, which may or may not contain the optimal policy. In \Cref{subsec:Preliminaries}, we stated that Assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg} hold for policies in $\Pi$ and we used this to argue that the Poisson equation has a solution given in \eqref{eq:PoissonEq}. As a result, repeating the  same arguments as in \Cref{thm:main} with the modification that $\pi^*_{\theta}$ is the best in-class policy of the MDP governed by parameter $\theta$, yields the following corollary. 

\begin{Corollary} \label{cor:main}
 Under Assumptions \ref{assump:costfn} through \ref{assump:sup_J_V},	the regret of \Cref{alg:TSDE} when using the best in-class policy is $\tilde O(d\sqrt{|\mathcal A|T})$. 
\end{Corollary}

\begin{Remark}\label{rem:irr}
 The derived regret bound can be extended to a larger class of MDPs which have transient states in addition to the single irreducible class. Specifically, for any $\theta_1,\theta_2 \in \Theta$, the Markov process with transition kernel $P_{\theta_1}^{\pi^*_{\theta_2}}$ obtained from the MDP $\left(\mathcal{X},\mathcal{A},c,P_{\theta_1}\right)$ by following policy $\pi^*_{\theta_2}$ has a single irreducible class $I_{\theta_1,\theta_2 }$ and a set of transient states $T_{\theta_1,\theta_2 }$. Furthermore, Assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg} hold for the single irreducible class. The reasoning behind the proof remains true in this case using the following argument: each episode $k$ starts at $0^d$, which is in the irreducible set for the chosen policy $\pi^*_{\theta_k}$, hence, throughout the episode, the algorithm remains in the irreducible set that is positive recurrent and never visits any transient states. In other words, episodes starting and ending at $0^d$ with a fixed episode-dependent policy implies that the reachable set of $0^d$ is all that can be explored, which is positive recurrent by our assumptions. As a result, we can restrict our proof derivations to the subset that is reachable from $0^d$ in each episode and follow the same analysis. The Lyapunov function-based bounds apply to the positive recurrent states, and hence, restricting attention to states reachable from $0^d$ within each episode, we can use these bounds for our assessment of regret using norms of the state. Thereafter, the coarse bounds on the norms of the state can be applied as carried out in our proof. \SAcomment{One example fitting this paradigm is the queueing system of \Cref{fig:QS1} with the optimal policy being a threshold policy. In \Cref{subsec:queue_1}, we show that Assumptions \ref{assump:costfn}-\ref{assump:sup_J_V} hold and \Cref{alg:TSDE} can be used to learn the optimal policy corresponding to the queueing system with unknown service rates.
 }
 
 %\vscomment{Mention that Example 1 fits the setting of this remark. When discussing Example 1 reminder the reader about this.}
\end{Remark}

\begin{Remark}\label{rem:oracle}
\SAcomment{\textbf{Requirement of an optimal policy oracle.}
To implement our algorithm, %when we determine regret with-respect-to an optimal policy, 
we need to find the optimal policy for each model sampled by the algorithm---optimal policy for \Cref{thm:main} and optimal policy within policy class $\Pi$ for \Cref{cor:main}; this has also been used in past work \cite{gopalan2015thompson,graves1997asymptotically,lai1995machine}. In the finite state-space setting, \cite{ouyang2017learning} provides a schedule of $\epsilon$ values and selects $\epsilon$-optimal policies to obtain $\tilde{O}(\sqrt{T})$ regret guarantees. The issue with extending the analysis of \cite{ouyang2017learning} to the countable state-space setting is that we need to ensure (uniform) ergodicity for the chosen $\epsilon$-optimal policies; the $\limsup$ or $\liminf$ of the time-average expected reward (used to define the average cost problem) being finite doesn't imply ergodicity. In other words, we must formulate (and verify) ergodicity assumptions for a potentially large set of close-to-optimal algorithms whose structure is undetermined. Another issue is that, to the best of our knowledge, there isn't a general structural characterization of all $\epsilon$-optimal stationary policies for countable state-space MDPs or even a characterization of the policy within this set that is selected by any computational procedure in the literature; current results only discuss existence and characterization of the stationary optimal policy. In the absence of such results, stability assumptions with the same uniformity across models as in our submission will be needed, which are likely too strong to be useful. %At present we don't know how to verify such an assumption for any example, but nevertheless the conditions required are likely to be too strong to be useful.

If we could verify the stability requirements of Assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg} for a subset of policies, the optimal oracle is not needed, and instead, by choosing approximately optimal policies within this subset, we can follow the same proof steps as \cite{ouyang2017learning} to guarantee regret performance similar to \Cref{cor:main} (without knowledge of model parameters). %To make this point clear, we assume that instead of the optimal policy, we have access to a (performance-wise) $\epsilon$-optimal policy and in \Cref{thm:Q2_eps_optimal}, we establish that the approximate policy satisfies the stability assumptions and the sub-linear regret bounds carry through following arguments similar to those in \cite[section 3.2]{ouyang2017learning}.
}
\end{Remark}

\SAcomment{To theoretically analyze the performance of the algorithm that follows an approximately optimal policy rather than the optimal one, we assume that for a specific sequence of $\{\epsilon_k\}_{k=1}^{\infty}$, an $\epsilon_k$-optimal policy is given, which is defined below. 
\begin{Definition}
   For each $\theta \in \Theta$, policy $\pi^{\epsilon}_\theta \in \Pi$ is called an $\epsilon$-optimal policy for model parameterized by $\theta$ if 
   $$ c(\boldsymbol x,\pi^\epsilon_\theta(\boldsymbol x))+  \sum_{\boldsymbol y \in \mathcal{X}} P_{\theta}(\boldsymbol y | \boldsymbol x,\pi^\epsilon_\theta(\boldsymbol x)) 	v(\boldsymbol y;\theta) \leq  c(\boldsymbol x,\pi^*_{\theta}(\boldsymbol x))+  \sum_{\boldsymbol y \in \mathcal{X}} P_{\theta}(\boldsymbol y | \boldsymbol x,\pi^*_{\theta}(\boldsymbol x)) 	v(\boldsymbol y;\theta)+\epsilon  ,$$ 
   where $\pi^*_{\theta}$ is the optimal policy in the policy class $\Pi$ corresponding to parameter $\theta$ and $v(.;\theta)$ is the solution to Poisson equation \eqref{eq:ACOE_case2}.
\end{Definition}
Given $\epsilon$-optimal policies that satisfy Assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg}, in \Cref{thm:Q2_eps_optimal} we extend the regret guarantees of \Cref{cor:main} to the algorithm employing  $\epsilon$-optimal policy,  instead of the best-in-class policy, and show that the same regret upper bounds continue to apply. The proof for \Cref{thm:Q2_eps_optimal} can be found in \Cref{subsec:proof_Q2_eps_optimal}.
 
\begin{Theorem}\label{thm:Q2_eps_optimal}
Consider a non-negative sequence $\{\epsilon_k\}_{k=1}^{\infty}$ such that for every $k \in \mathbb{N}$, $\epsilon_k$ is bounded above by  $\frac{1}{k+1}$ and an $\epsilon_k$-optimal policy satisfying Assumptions \ref{assump:geom_erg} and \ref{assump:poly_erg} is given.
 The regret incurred by \Cref{alg:TSDE} while using the $\epsilon_k$-optimal policy during any episode $k$ is $\tilde O(d\sqrt{|\mathcal A|T})$. 
\end{Theorem}
}

==> Simulations.tex <==
% \section{Evaluation: Application of \texorpdfstring{\Cref{alg:TSDE}}{Algorithm 1} to queueing models}

\section{Evaluation: Application of \Cref{alg:TSDE} to queueing models}
\label{sec:evaluation}

%\vscomment{We had discussed other algorithms as comparison in the summer. None of those are present in the current draft. Also, can you try to find empirically the polynomial dependence in $T$ of the regret for these two examples?}  
Next, we present an evaluation of our algorithm. We study two different queueing models shown in \Cref{fig:QS}, each with Poisson arrivals at rate $\lambda$, and two heterogeneous servers with exponentially distributed services times with unknown service rate vector $\boldsymbol \theta^*=(\theta_1^*, \theta_2^*)$. 
Vector $\boldsymbol \theta^*$ is sampled from the prior distribution $\nu$ defined on the space $\Theta$ given as
\begin{equation*}
	\Theta= \Big\{(\theta_1,\theta_2) \in {\R}_+^2: \frac{\lambda}{\theta_1+\theta_2} \leq \frac{1-\delta}{1+\delta}, 1 \leq \frac{\theta_1}{\theta_2} \leq R \Big\},
\end{equation*} for fixed $R\geq 1$ and $\delta \in (0,0.5)$. The first condition ensures the stability of the queueing models, while the second condition  guarantees the compactness of the parameter space of the parameterized policies. In both systems, the goal of the dispatcher is to minimize the expected sojourn time of the jobs, which by Little's law \cite{srikant2013communication} is equivalent to minimizing the average number of jobs in the system. After verifying Assumptions \ref{assump:costfn}-\ref{assump:sup_J_V} in \Cref{sec:queueing_models} for the cost function $c(\boldsymbol x,a)= \norm{\boldsymbol x}_1$, \Cref{thm:main} yields a  Bayesian regret of order $\tilde O(\sqrt{T})$ for \Cref{alg:TSDE}.

\textit{\bfseries Model 1: Two-server queueing system with a common buffer.} 
We consider the continuous-time queueing system of \Cref{fig:QS1}, where the  countable state space is
$\mathcal{X}=\{\boldsymbol x=(x_0,x_1,x_2)\in \mathbb{Z}_+ \times \{ 0,1\}^2\}$, where $x_0$ is the queue length, and $x_i$, $i=1,2$ equal $1$ if server $i$ is busy. The action space is $\mathcal{A}=\{h, b, 1,2\}$, where $h$ means no action, $b$ sends a job to both servers, and $i=1,2$ assigns a job to server $i$. In \cite{lin1984optimal}, it is shown that by uniformization \cite{lippman1975applying}
and sampling the continuous-time Markov process at rate $\lambda+\theta_1^*+ \theta_2^*$, a discrete-time MDP is obtained, which converts the original continuous-time  problem to an equivalent discrete-time problem where we need to minimize $\limsup_{T\rightarrow\infty} T^{-1} \sum_{t=0}^{T-1}  \norm{\boldsymbol{X}(t)}_1$.	 
Further, \cite{lin1984optimal} shows that the optimal policy achieving the infimum average number of jobs
is a threshold policy $\pi_{t(\boldsymbol \theta^*)}$ with optimal finite threshold $t(\boldsymbol \theta^*) \in \mathbb{N}$: always assign a job to the faster (first) server when free, and to the second server if it is free and $\norm{\boldsymbol x}_1 >t(\boldsymbol \theta^*)$, and take no action otherwise.  
In \Cref{subsec:queue_1}, we argue that the discrete-time Markov process governed by $\theta \in \Theta$ and following threshold policy $\pi_t$ for a set of optimal thresholds $t$ being bounded satisfies Assumptions \ref{assump:costfn}-\ref{assump:sup_J_V}.



	% \begin{figure*}[t]
	% \centering
	% \subfloat[Queueing system with a common buffer.  \label{fig:QS1}]{\includegraphics[width=0.43\linewidth]{Figures/QS1.pdf}} \hspace{1cm}
	% \subfloat[Two parallel queues.  \label{fig:QS2}]{\includegraphics[width=0.4\linewidth]{Figures/QS2.pdf}}
	% \caption{Two-server queueing systems with heterogeneous service rates.
	% }
	%  \label{fig:QS}
	% \end{figure*}




\begin{figure}[t]
    \centering
    \begin{subfigure}{0.43\textwidth}
        \centering
        {\includegraphics[width=1\linewidth]{QS1.pdf}}
        \caption{Queueing system with a common buffer.}
        \label{fig:QS1}
    \end{subfigure}\hspace{0.5cm}
    \begin{subfigure}{0.4\textwidth}
        \centering
        {\includegraphics[width=1\linewidth]{QS2.pdf}}
        \caption{Two parallel queues.}
        \label{fig:QS2}
    \end{subfigure}%
    \caption{Two-server queueing systems with heterogeneous service rates.}
    \label{fig:QS}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.43\textwidth}
        \centering
        {\includegraphics[width=1\linewidth]{M1.png}}
        \caption{Queueing system of \Cref{fig:QS1}.}
        \label{fig:regret_QS1}
    \end{subfigure}\hspace{1cm}
    \begin{subfigure}{0.43\textwidth}
        \centering
        {\includegraphics[width=1\linewidth]{M2.png}}
        \caption{Queueing system of \Cref{fig:QS2}.}
        \label{fig:regret_QS2}
    \end{subfigure}%
    \caption{Regret performance for $\lambda=0.3,0.5,0.7$. Shaded region shows the  $\pm \sigma$ area of mean regret.}
    \label{fig:regret}
\end{figure}




\textit{\bfseries Model 2: Two heterogeneous parallel queues.} 
We consider the continuous-time queueing system of \Cref{fig:QS2} with   countable state space
$\mathcal{X}=\{\boldsymbol x =(x_1,x_2)\in \mathbb{Z}_+^2 \}$, where 
$x_i$ is the number of jobs in the server-queue pair $i$. The action space is $\mathcal{A}=\{ 1,2\}$,
where action $i$ sends the arrival to queue $i$. We obtain the discrete-time MDP by sampling the queueing system at the arrivals, and then aim to find the average cost minimizing policy within the class 
$\Pi=\{\pi_{\omega}; {\omega}\in [(c_RR)^{-1},c_RR]\}$, 
$c_R \geq 1$. Policy $\pi_{\omega} : \X \rightarrow \mathcal A$ routes arrivals based on the weighted queue lengths:
$\pi_{\omega} (\boldsymbol x)=\argmin \left(1+x_1,{\omega} \left(1+x_2\right)\right)$ with ties broken for $1$. 
Even with the transition kernel fully specified (by the values of arrival  and service rates), the optimal policy  
in $\Pi$ is not known except when $\theta_1=\theta_2$ where the optimal value is ${\omega}=1$, and so, to learn it, we will use Proximal Policy Optimization with approximating martingale-process (AMP) method for countable state space MDPs~\cite{dai2022queueing}. 
Note that \cite{dai2022queueing} requires full model knowledge, which holds within our scheme as we use parameters sampled from the posterior for guessing the true model and then select the policy at the beginning of each episode---the parameters sampled from the posterior are assumed to yield the true model for execution in each phase. In \Cref{subsec:queue_2}, we argue that the discrete-time Markov process governed by parameter $\theta \in \Theta$ and following policy $\pi_{\omega}$ for $\omega \in[(c_RR)^{-1},c_RR]$ satisfies Assumptions \ref{assump:costfn}-\ref{assump:sup_J_V}.

Next, we report the numerical results of \Cref{alg:TSDE}  in the two queueing models of \Cref{fig:QS} and calculate regret using \eqref{eq:regret_def}. The regret is averaged over 2000 simulation runs and plotted against the number of transitions in the sampled discrete-time Markov process. \Cref{fig:regret} shows the behavior of the regret of the two queueing models for three different arrival rates and service rates distributed according to a Dirichlet prior over $ [0.5,1.9]^2$.
For the queueing model of \Cref{fig:QS1}, the minimum average cost $J(\theta)$ and optimal policy $\pi^*_{\theta}$ are known explicitly~\cite{lin1984optimal} for every $\theta \in \Theta$, which are used in \Cref{alg:TSDE} and for regret calculation. Conversely, for the second queueing model, $J(\theta)$ and $\pi^*_{\theta}$ are not known and the PPO algorithm~\cite{dai2022queueing} is used to empirically find both the optimal weight and the policy's average cost. 
Additional details of the simulations and more plots are presented in \Cref{sec:num_res}.
\SAcomment{As expected from our theoretical guarantees, we observe that the regret is sub-linear in time.  Furthermore, it grows as the arrival rate increases and the normalized load on the system converges to $1$, which is expected since the system gets closer to the stability boundary. As discussed in \Cref{sec:main_results},  our bound on the expected regret is linearly dependent on $J^*$ and, thus, will increase with the arrival rate, reinforcing the previous comment.}


\section{Conclusions and future work}

We studied the problem of learning optimal policies in countable state space MDPs governed by unknown parameters. We proposed a learning policy based on Thompson sampling and established finite-time performance guarantees for the Bayesian regret. We highlighted the practicality of our proposed algorithm by considering two different queueing models with unknown service rates and showing that our algorithm can be applied to develop optimal control policies. Specifically, we argued that for two different queueing models, the ergodicity assumptions of our algorithm are satisfied, and we further numerically investigated the regret performance of our algorithm. For future work, we plan to extend the applicability of our algorithm to a broader class of problem settings and generalize it to consider policies that do not necessarily ensure stability. Additionally, we aim to simplify our proposed algorithm by incorporating ideas from \cite{theocharous2018scalar}.

\section*{Disclosure of Funding}
SA's research was supported by NSF via grants ECCS2038416, CCF2008130, and CNS1955777, and a grant from General Dynamics via MIDAS at the University of Michigan, Ann Arbor. VS's research is supported by NSF via grants ECCS2038416, CCF2008130, CNS1955777, and CMMI2240981.
